Learning to Execute Actions or Ask Clarification Questions

Collaborative tasks are ubiquitous activities where a form of communication is required in order to reach a joint goal. Collaborative building is one of such tasks. We wish to develop an intelligent builder agent in a simulated building environment (Minecraft) that can build whatever users wish to build by just talking to the agent. In order to achieve this goal, such agents need to be able to take the initiative by asking clarification questions when further information is needed. Existing works on Minecraft Corpus Dataset only learn to execute instructions neglecting the importance of asking for clarifications. In this paper, we extend the Minecraft Corpus Dataset by annotating all builder utterances into eight types, including clarification questions, and propose a new builder agent model capable of determining when to ask or execute instructions. Experimental results show that our model achieves state-of-the-art performance on the collaborative building task with a substantial improvement. We also define two new tasks, the learning to ask task and the joint learning task. The latter consists of solving both collaborating building and learning to ask tasks jointly.

==> paper/analysis.tex <==
Although our model can perform better that the baselines, it is still challenging for our model to the whole action sequence correctly. In Figure \ref{fig:case}, the architect instructed the builder to build a 3x3 square. Although our model can predict parts of actions correctly, it fails to complete all required actions in the action sequence.

Meanwhile, some other factors also make the learning process more challenging. Firstly, builder action sequences are noisy caused by, for example, the accidentally clicking in the generation process.

